Estimating Neural Reflectance Field from Radiance Field using Tree Structures

We present a new method for estimating the Neural Reflectance Field (NReF) of an object from a set of posed multi-view images under unknown lighting. NReF represents 3D geometry and appearance of objects in a disentangled manner, and are hard to be estimated from images only. Our method solves this problem by exploiting the Neural Radiance Field (NeRF) as a proxy representation, from which we perform further decomposition. A high-quality NeRF decomposition relies on good geometry information extraction as well as good prior terms to properly resolve ambiguities between different components. To extract high-quality geometry information from radiance fields, we re-design a new ray-casting based method for surface point extraction. To efficiently compute and apply prior terms, we convert different prior terms into different type of filter operations on the surface extracted from radiance field. We then employ two type of auxiliary data structures, namely Gaussian KD-tree and octree, to support fast querying of surface points and efficient computation of surface filters during training. Based on this, we design a multi-stage decomposition optimization pipeline for estimating neural reflectance field from neural radiance fields. Extensive experiments show our method outperforms other state-of-the-art methods on different data, and enable high-quality free-view relighting as well as material editing tasks.

==> figures/fig_application.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.15\linewidth]{images/albedo_ours.png}~
    \includegraphics[width=0.15\linewidth]{images/normal_our_refine.png}
    \includegraphics[width=0.15\linewidth]{images/render_our.png}~
    \includegraphics[width=0.15\linewidth]{images/render_our.png}~
    \includegraphics[width=0.15\linewidth]{images/render_our.png}
    
    \includegraphics[width=0.15\linewidth]{images/albedo_nosparse.png}~
    \includegraphics[width=0.15\linewidth]{images/normal_NeRFactor.png}~
    \includegraphics[width=0.15\linewidth]{images/render_nosparse.png}~
    \includegraphics[width=0.15\linewidth]{images/render_nosparse.png}~
    \includegraphics[width=0.15\linewidth]{images/render_nosparse.png}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Application, from left to right, albedo, normal, render, novel lighting, novel lighting}
    \label{fig:application}
\end{figure*}

==> figures/fig_method_overview.tex <==
\begin{figure}[!ht]
     \centering
     \includegraphics[width=0.45\textwidth]{images/method.pdf}
%     \setlength{\abovecaptionskip}{pt}
     \setlength{\belowcaptionskip}{-10pt}
     \caption{Our optimization pipeline for NReF estimation. We first extract an initial surface from a NeRF (green). Then we construct an ``memory bank" (gray) which stores discrete NReF samples on surface points and accelerate it with multiple data structures. The memory bank enables a alternating optimization process: a ``local" step (blue) updates NReF with render loss and commitment w.r.t memory bank, and a ``global" step (orange) updates memory bank by applying a set of priors.}
     \label{fig:method_overview}
\end{figure}

==> figures/fig_method_visibility.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\linewidth]{images/vis_handle.png}
     \setlength{\abovecaptionskip}{-2pt}
     \setlength{\belowcaptionskip}{-10pt}    
    \caption{Handelling visibility in pretrain}
    \label{fig:vis_handle}
\end{figure}

